Vector Quantile Regression on Manifolds

Quantile regression (QR) is a statistical tool for distribution-free estimation of conditional quantiles of a target variable given explanatory features. QR is limited by the assumption that the target distribution is univariate and defined on an Euclidean domain. Although the notion of quantiles was recently extended to multi-variate distributions, QR for multi-variate distributions on manifolds remains underexplored, even though many important applications inherently involve data distributed on, e.g., spheres (climate and geological phenomena), and tori (dihedral angles in proteins). By leveraging optimal transport theory and c-concave functions, we meaningfully define conditional vector quantile functions of high-dimensional variables on manifolds (M-CVQFs). Our approach allows for quantile estimation, regression, and computation of conditional confidence sets and likelihoods. We demonstrate the approach's efficacy and provide insights regarding the meaning of non-Euclidean quantiles through synthetic and real data experiments.

==> figs/contour_vqe.tex <==
\newcommand\wc{0.32\linewidth}
\newcommand\midw{\hspace{0.6cm}}
\newcommand{\emptyim}[0]{\hfill\begin{subfigure}[b]{0.3\linewidth}
\end{subfigure}}
\newcommand\sw{0.75\linewidth}
\newcommand\tw{1\linewidth}

% horizontal layout
\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{0.6\linewidth}
%% s2 base
\begin{subfigure}[b]{\wc}
\centering
\begin{overpic}
[trim=0cm 0cm 0cm 0cm,clip,width=\sw, grid=false]{./figs/manifolds/base_s2.pdf}
\put(-34,30){\rotatebox{90}{Sphere}}
\put(26,100){Uniform}
\end{overpic}
% \caption{\label{fig:cont_base_s2} Base}
\end{subfigure} 
\hfill
%% s2 heart
\begin{subfigure}[b]{\wc}
\centering
\begin{overpic}
[trim=38.5cm 12cm 5.5cm 6cm,clip,width=\sw, grid=false]{./figs/manifolds/heart_s2_cont.pdf}
\put(35,100){Heart}
\put(80,2){\tiny 0.65}
\end{overpic}
% \caption{\label{fig:cont_heart_s2} Heart}
\end{subfigure}
\hfill 
%% s2 star
\begin{subfigure}[b]{\wc}
\centering
\begin{overpic}
[trim=38.5cm 12cm 5.5cm 6cm,clip,width=\sw, grid=false]{./figs/manifolds/star_s2_cont.pdf}
\put(35,100){Star}
\put(80,2){\tiny 0.31}
\end{overpic}
% \caption{\label{fig:cont_star_s2} Star}
\end{subfigure}
%% legend
% \begin{subfigure}[t]{0.1\linewidth}
% \begin{overpic}
% [trim=0cm 0cm 0cm 0cm,clip,width=0.3\linewidth, grid=false]{./figs/manifolds/legend_cont}
% \end{overpic}
% \end{subfigure}
\\
%% torus base
\begin{subfigure}[b]{\wc}
\centering
\begin{overpic}
[trim=0cm 0cm 0cm 0cm,clip,width=\tw, grid=false]{./figs/manifolds/base_torus.pdf}
\put(-10,20){\rotatebox{90}{Torus}}
\end{overpic}
% \caption{\label{fig:cont_base_torus} Base}
\end{subfigure}
\hfill 
%% torus heart
\begin{subfigure}[b]{\wc}
\centering
\begin{overpic}
[trim=0cm 0cm 0cm 0cm,clip,width=\tw, grid=false]{./figs/manifolds/heart_torus_cont.pdf}
\put(80,2){\tiny 0.6}
\end{overpic}
% \caption{\label{fig:cont_heart_torus} Heart}
\end{subfigure}
\hfill 
%% torus star
\begin{subfigure}[b]{\wc}
\centering
\begin{overpic}
[trim=0cm 0cm 0cm 0cm,clip,width=\tw, grid=false]{./figs/manifolds/star_torus_cont.pdf}
\put(91,91){\includegraphics[scale=0.2]{figs/manifolds/legend_cont.pdf}}
\put(97,140){\scriptsize $\tau$}
\put(80,2){\tiny 0.62}
\end{overpic}
% \caption{\label{fig:cont_star_torus} Star}
\end{subfigure}

\caption{\label{fig:vqe_cont}  $\tau$-contours}
\end{subfigure}
\hspace{0.4cm}
%% coverages
\begin{subfigure}[b]{0.3\linewidth}
\centering
    \begin{overpic}
[trim=0.6cm 1.2cm 4.4cm 2cm, clip, width=0.9\linewidth, grid=false]{./figs/manifolds/coverage}
\put(-2,40){\rotatebox[origin=c]{90}{\tiny 
 Mean coverage}}
 \put(50,-1){\footnotesize $\tau$}

 \put(100,64){\tiny Nominal}
  \put(100,59){\tiny $\Sphere{2}$ star}
  \put(100,54){\tiny $\Sphere{2}$ heart}
  \put(100,48.5){\tiny $\mathcal{T}$ star}
  \put(100,43.5){\tiny $\mathcal{T}$ heart}
\end{overpic}
\vspace{0.7cm}
\caption{\label{fig:vqe_cov} Mean coverages}
\end{subfigure}
\caption{\label{fig:vqe_cont_cov}
\textbf{$\tau$-contours of unconditional heart- and star-shaped distributions accurately estimated on $\cset{S}^2$ and $\cset{T}$}.
\emph{Left:} Estimated $\tau$-contours, each containing $100\cdot\tau$ percent of the data plotted over the ground truth data.
Shown are the contours in the base uniform distribution (rotated for visual clarity), and the target heart- and star-shaped distributions. For the latter two, we report the KDE-$L_1$ loss ($\times 10^{-5}$).
\emph{Right:} The obtained mean coverage on the Heart and Star distributions closely matches the desired nominal coverage.
}
\end{figure*}



%vertical layout
% \begin{figure}[t!]
% \centering
% \begin{subfigure}[b]{\wc}
% \centering
% \begin{overpic}
% [trim=0cm 0cm 0cm 0cm,clip,width=\sw, grid=false]{./figs/manifolds/base_s2.pdf}
% \put(-12,30){\rotatebox{90}{Uniform}}
% \put(34,100){Sphere}
% \end{overpic}
% % \caption{\label{fig:cont_base_s2} Base}
% \end{subfigure}
% \midw
% %% torus base
% \begin{subfigure}[b]{\wc}
% \centering
% \begin{overpic}
% [trim=0cm 0cm 0cm 0cm,clip,width=\tw, grid=false]{./figs/manifolds/base_torus.pdf}
% \put(37,74){{Torus}}
% \put(99,20){\includegraphics[scale=.04]{figs/manifolds/legend_cont.png}}
% \put(104,59){\scriptsize $\tau$}
% \end{overpic}
% % \caption{\label{fig:cont_base_torus} Base}
% \end{subfigure}
% %% s2 heart
% \begin{subfigure}[b]{\wc}
% \centering
% \begin{overpic}
% [trim=37.5cm 11cm 5cm 5cm,clip,width=\sw, grid=false]{./figs/manifolds/heart_s2_cont.pdf}
% \put(-12,33){\rotatebox{90}{Heart}}
% \end{overpic}
% % \caption{\label{fig:cont_heart_s2} Heart}
% \end{subfigure}
% \midw
% %% torus heart
% \begin{subfigure}[b]{\wc}
% \centering
% \begin{overpic}
% [trim=0cm 0cm 0cm 0cm,clip,width=\tw, grid=false]{./figs/manifolds/heart_torus_cont.pdf}
% \end{overpic}
% % \caption{\label{fig:cont_heart_torus} Heart}
% \end{subfigure}
% %% s2 star
% \begin{subfigure}[b]{\wc}
% \centering
% \begin{overpic}
% [trim=37.5cm 11cm 5cm 5cm,clip,width=\sw, grid=false]{./figs/manifolds/star_s2_cont.pdf}
% \put(-12,36){\rotatebox{90}{Star}}
% \end{overpic}
% % \caption{\label{fig:cont_star_s2} Star}
% \end{subfigure}
% \midw
% % torus star
% \begin{subfigure}[b]{\wc}
% \centering
% \begin{overpic}
% [trim=0cm 0cm 0cm 0cm,clip,width=\tw, grid=false]{./figs/manifolds/star_torus_cont.pdf}
% \end{overpic}
% % \caption{\label{fig:cont_star_torus} Star}
% \end{subfigure}

% \caption{\label{fig:vqe_cont} $\tau$-contours of multiple distributions plotted on the sphere and torus. Different colours correspond to $\tau$-contours, each containing  $\tau$ percentage of the data. }
% \end{figure}



==> figs/kde_codon.tex <==
\newcommand\wc{0.3\linewidth}
%%% TEST FIGURES %%%
\begin{figure*}[h!]
\centering
%% s2 base
\begin{subfigure}[b]{\wc}
\centering
\begin{overpic}
[trim=2.07cm 2.05cm 3cm 3cm,clip,width=\linewidth, grid=False]{./figs/manifolds/kde_flat_G.pdf}
\put(4,37){\tiny Ground truth}
\put(63,37){\tiny Estimated}
\end{overpic}
\caption{\label{fig:kde_G} G}
\end{subfigure} 
\hfill
\begin{subfigure}[b]{\wc}
\centering
\begin{overpic}
[trim=2.07cm 2.05cm 3cm 3cm,clip,width=\linewidth, grid=false]{./figs/manifolds/kde_flat_N.pdf}
\put(4,37){\tiny Ground truth}
\put(63,37){\tiny Estimated}
\end{overpic}
\caption{\label{fig:kde_N} N}
\end{subfigure} 
\hfill
\begin{subfigure}[b]{\wc}
\centering
\begin{overpic}
[trim=2.07cm 2.05cm 3cm 3cm,clip,width=\linewidth, grid=false]{./figs/manifolds/kde_flat_P.pdf}
\put(4,37){\tiny Ground truth}
\put(63,37){\tiny Estimated}
\end{overpic}
\caption{\label{fig:kde_P} P}
\end{subfigure} 
\caption{\label{fig:kde_codon}}
\end{figure*}

==> figs/vqe_coverage.tex <==
\begin{figure}[t]
\centering
\hspace{0.08\linewidth}
\begin{subfigure}[b]{0.7\linewidth}
\centering
    \begin{overpic}
[trim=0.6cm 1.2cm 4.4cm 2cm, clip, width=0.9\linewidth, grid=false]{./figs/manifolds/coverage}
\put(-1,40){\rotatebox[origin=c]{90}{\tiny 
 Mean coverage}}
 \put(50,0){\footnotesize $\tau$}

 \put(100,64){\scriptsize Nominal}
  \put(100,59){\scriptsize $\Sphere{2}$ star}
  \put(100,54){\scriptsize $\Sphere{2}$ heart}
  \put(100,48.5){\scriptsize $\mathcal{T}$ star}
  \put(100,43.5){\scriptsize $\mathcal{T}$ heart}
\end{overpic}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.05\linewidth}
\end{subfigure}
\caption{\label{fig:cov_vqe} Mean coverage of $\tau$-contours computed in Figure \ref{fig:vqe_cont}.}
\end{figure}


==> figs/vqr_kde.tex <==
\begin{figure*}[t]
\centering
\begin{overpic}
[trim=0cm 1.85cm 0cm 0cm,clip, width=1\linewidth, grid=false]{./figs/manifolds/kde_vqr}
% s2 heart
\put(5,32.5){\footnotesize GT}
\put(12.5,32.5){\footnotesize Estimated}
\put(20.8,22){\scriptsize 1.43}
\put(20.8,11.5){\scriptsize 0.84}
\put(20.8,1){\scriptsize 1.43}
% \put(20.8,1){\scriptsize 2.01}
% s2 star
\put(27,32.5){\footnotesize GT}
\put(34.5,32.5){\footnotesize Estimated}
\put(42.8,22){\scriptsize 0.83}
\put(42.8,11.5){\scriptsize 0.84}
\put(42.8,1){\scriptsize 1.28}
% \put(42.8,1){\scriptsize 1.91}
% torus heart
\put(50.5,32.5){\footnotesize GT}
\put(61,32.5){\footnotesize Estimated}
\put(70,22){\scriptsize 2.99}
\put(70,11.5){\scriptsize 1.85}
\put(70,1){\scriptsize 2.3}
% \put(70,1){\scriptsize 2.62}
% torus star
\put(77.5,32.5){\footnotesize GT}
\put(88.5,32.5){\footnotesize Estimated}
\put(97.5,22){\scriptsize 3.28}
\put(97.5,11.5){\scriptsize 1.6}
\put(97.5,1){\scriptsize 2.41}
% \put(97.5,1){\scriptsize 3.26}
% conditioning
\put(0,24){\rotatebox{90}{\scriptsize $x=0.7$}}
\put(0,14){\rotatebox{90}{\scriptsize $x=1$}}
\put(0,3){\rotatebox{90}{\scriptsize $x=1.3$}}
% \put(0,2){\rotatebox{90}{\scriptsize $x=1.7$}}
\end{overpic}
\caption{\label{fig:kde_vqr}
\textbf{Reconstruction of distribution $\rvec{Y}|\rvec{X}$ using the estimated M-CVQF.}
We also report the KDEL-L1 loss for different conditioning. All the values are multiplied by $10^{-5}$.}
\end{figure*}

